Safe Connectivity Maintenance of Underactuated Multi-Agent Networks in Dynamic Oceanic Environments

Autonomous multi-agent systems are increasingly being deployed in environments where winds and ocean currents have a significant influence. Recent work has developed control policies for single agents that leverage flows to achieve their objectives in dynamic environments. However, in multi-agent systems, these flows can cause agents to collide or drift apart and lose direct inter-agent communications, especially when agents have low propulsion capabilities. To address these challenges, we propose a hierarchical multi-agent control approach that allows arbitrary single-agent performance policies that are unaware of other agents to be used in multi-agent systems while ensuring safe operation. We first develop a safety controller using potential functions, solely dedicated to avoiding collisions and maintaining inter-agent communication. Next, we design a low-interference safe interaction (LISIC) policy that trades off the performance policy and the safety control to ensure safe and performant operation. Specifically, when the agents are at an appropriate distance, LISIC prioritizes the performance policy while smoothly increasing the safety controller when necessary. We prove that under mild assumptions on the flows experienced by the agents, our approach can guarantee safety. Additionally, we demonstrate the effectiveness of our method in realistic settings through an extensive empirical analysis with simulations of fleets of underactuated autonomous surface vehicles operating in dynamic ocean currents where these assumptions do not always hold.

==> xx_lit_review.tex <==
\label{sec:lit_review}

Control of \ac{MAS} is a vast topic, where methods to attempt maintaining connectivity have spanned from graph theoretic methods \cite{mesbahiGraphTheoreticMethods2010}, to flocking \cite{olfati-saberFlockingMultiAgentDynamic2006} \cite{zavlanosPotentialFieldsMaintaining2007} \cite{zavlanosFlockingPreservingNetwork2007} and more recently to \ac{MPC} \cite{filotheouDecentralizedControlUncertain2018} \cite{carron2023multi} and learning approaches \cite{riviereGLASGlobaltoLocalSafe2020a}. Navigating multi-agent networks in complex flows while maintaining connectivity can be interpreted as a cooperative or collective task where popular methods for multi-agent include formation control, coverage control, containment control or flocking to name a few of them \cite{chenControlMultiAgentSystems2019}. Nevertheless, only a flocking-inspired behavior seems relevant to this work, as enforcing a specific geometric shape for formation control would not leverage any particular synergy. In this context, the objective of maintaining connectivity and avoiding collisions is purely distance-based. Flocking has been applied successfully to unmanned aerial vehicles (UAVs), autonomous robots and multi-agent systems. Interestingly, flocking is nature-inspired from birds flocks, schools of fishes without any central unit coordinator \cite{zavlanosFlockingPreservingNetwork2007}. Flocking algorithms generally embody the three heuristic rules of Reynolds, known as flock centering, collision avoidance and velocity matching \cite{olfati-saberFlockingMultiAgentDynamic2006}. In this work, we focus on the setting where the multi-agent objective can be decomposed into single agent objectives that can be optimized independently. For example, in floating seaweed farms, the seaweed growth of each agent does not depend on the growth of other agents. As a state-space system implication, this means the multi-agent system is not strictly interconnected i.e. the state of each agent does not depend on the other agent states of the system. However, in such applications the agents are still coupled by constraints, such as not colliding with each other and maintaining inter-agent connectivity. This motivates a hierarchical approach to decompose the objective into two simpler, smaller problems, similar to hierarchical reinforcement learning principles \cite{pateriaHierarchicalReinforcementLearning2021}. \ac{H-MAS} have foremost seen application to smart control of microgrid systems \cite{douMultiAgentBasedHierarchical2013} or control of modular multilevel converters \cite{drekeConsensusHierarchicalMultiagent2022}.
Although not explicitly listed as a hierarchical approach, \cite{lollaPathPlanningMultiscale2015} solves path planning and ocean vehicles coordination separately with a leader-follower description. Especially relevant is the similar context of limited-speed vehicles sensitive to ocean currents, where dynamic formation control intrinsically accounts for connectivity maintenance and collision avoidance. Nevertheless, the use of optimization techniques to enforce regular polygon formations could reveal quite conservative and increase the complexity for the solely distance-based constraints of this work. In this context of \ac{H-MAS}, a performance controller is assumed to be known for each agent and the goal is to minimally interfere with the individual agent objective while maintaining connectivity and collision avoidance. For example, a time-optimal control to a target is available for each agent and constraint satisfaction should be traded-off intelligently with the performance objective.\\
In most of the above literature based on reactive or flocking approaches, simple integrator or double integrator are considered. However, in realistic scenarios such as ocean navigation, the agents are subject to non-linear time varying dynamics and small autonomous vessels are often under-actuated. Therefore, disconnections are sometimes not avoidable and the multi-agent scheme need to be resilient and able to achieve connectivity. As local communication are to be maintained, a flock configuration maintaining an ideal distance between agents is of particular interest. In this work, we propose a flocking-inspired multi-agent control approach blending a nominal performance single agent control with constraint violation penalization using potential fields \cite{zavlanosPotentialFieldsMaintaining2007}. While flocking robustness and adaptability have been extended to more challenging environments with non-linearities and parameter uncertainties under certain assumptions \cite{yuRobustAdaptiveFlocking2010a}, \cite{wangFlockingMultipleAutonomous2013} \cite{zhangAdaptiveFlockingNonlinear2015} \cite{zouFlockingUncertainNonlinear2021}, it is rarely combined with under-actuated agents. Some adaptive flocking control method handling under-actuation have considered approximating the uncertain nonlinear dynamics through RBF Neural Networks \cite{pengNeuralAdaptiveFlocking2012}. However, learning approaches for approximating the uncertain dynamics are more challenging when only sparse data is available along a grid, such as for ocean forecasts. Additionally, if the performance controller is a planning algorithm \cite{wiggert_etal_CDC2022}, it might be also subject to uncertainty due to forecast error and lack of realistic distribution of the flows.
Therefore, we stress the importance of our approach for recovery abilities in case of connectivity failures, as the communication network evolves over time. The dynamics of communication and information sharing could then later be handled on a another level with a Plug-and-Play control scheme \cite{PnP}, but is not in the focus of this work.
We demonstrate our control hierarchy in realistic, challenging non-linear, under-actuated dynamics and compare controllers empirically. Performance is quantified in terms of connectivity quality, the performance objective satisfaction, and the recovery abilities in case of connectivity failures. \\






In this section, we describe the relevant literature spanning
The related work consists of
\mwnote{Lots of great related work! It's definitly way too much for the paper, needs to be clustered/shortened to the key aspects/differences to us. For the thesis write it out more. The structure I like most for Introduction is: Motivation (what is the problem in words), then related work (what have others done to solve similar problems), then what is our contribution and how does it with with existing work. Maybe that helps to prioritize which aspects to keep.}
%\begin{itemize}
\subsection{Multi-Agent Systems background:} 
    \begin{itemize}
        \item \cite{bulloDistributedControlRobotic2009}, survey on the control of multi-agents with formation control, consensus, pairwise connectivity maintenance problem, using pairwise connectivity constraint set, rendezvous algorithm \cite{chenControlMultiAgentSystems2019}
        \item Usage of Reachability, Level Set Method in non linear complex flows but for formation control of ocean surface vessels \cite{lollaPathPlanningMultiscale2015}
        \item Multi Agent network analysis based on graph theory. Interesting because chapter 7 introduces mobile robots an $\Delta$ disk proximity graph, and cooperative dynamics (limited to single integrator, linear, no uncertainty). Propose decentralized control laws for \textbf{dynamic graphs} (graph chaing as the agents move in and out of each other's sensory range). Indicator value to know whether two agents are connected, weighted graph-based feedback. Similar to \textbf{flocking}, presents decentralized control laws over neighbors as a function of the edge tension. Raises a total tension energy of the graph \cite{mesbahiGraphTheoreticMethods2010}.
        \item Base Paper for our reactive control approach, (again the notion of pairwise connectivity introduced in \cite{bulloDistributedControlRobotic2009}. Decentralized, communication and collision avoidance while leading each robot to their (individual goal), but single integrator dynamics (linear). Hard switching between modes (achieve connectivity, maintain connectivity, navigate towards the goal) \cite{pereiraDecentralizedMotionPlanning}
        \item Work on connectivity maintenance, proximity-based communication models (e.g. disk based). Employs adjacency and Laplacian matrix and spectral properties. Centralized or distributed algorithms approaches to maintain, increase control connectivity in mobile robot networks. Approaches with convex optimization, subgradient-descent to maximize algebraic connectivity, but also potential fields. Application to rendezvous, flocking and formation control \cite{zavlanosGraphtheoreticConnectivityControl2011a}
        \item Approach based on "k-hop" connectivity, centralized control framework guaranteeing graph connectivity at all time. algebraic model for connectivity: k-connectivity matrix that captures the connectivity property of a graph.\cite{zavlanosControllingConnectivityDynamic2005}, 
        \item BUT none of them address non linear dynamics and underactuated setting
    \end{itemize}

    %%
\subsection{Flocking behaviour:}
    \begin{itemize}
        \item Base paper for flocking  \cite{olfati-saberFlockingMultiAgentDynamic2006}
        \item Notion of artificial potential fields. Connectivity condition is translated to differentiable constraints on individual agent motion by considering the dynamcis of the Laplacian matrix and its spectral properties: \cite{zavlanosPotentialFieldsMaintaining2007}
        \item Use flocking for network that change arbitrarily (no dwell time between consecutive switches), guarantee stabilization of inter-agent distances with flocking \cite{tannerFlockingFixedSwitching2007a}
    \end{itemize}

    %%
\subsection{Flocking with NonLinear/Robust approaches:}
  Here all are listed for 2nd order systems. Generally have a velocity matching term that is modified to account for nonlinearities or disturbances. We dont have a velocity matching term as our dynamics are first order (but our flocking control could be extended with one of their approach if the system was 2nd order)
    \begin{itemize}
        \item Nonlinear dynamics, agent coupling weights are perturbed by asymmetric uncertain parameters. \cite{yuRobustAdaptiveFlocking2010a}
        \item Flocking with heterogeneous non linear dynamics, while enabling agents to move with same velocity. mild assumption that initial network should be connected. Nonlinear dynamical single virtual leader \cite{wangFlockingMultipleAutonomous2013}
        \item Adaptive Flocking with uncertain parameters.  Design adaptvie flocking of nonlinear multi agents systems with uncertain parameters
        \cite{zhangAdaptiveFlockingNonlinear2015}
        \item Robust Flocking for 2nd order non linear systems with a leader and external disturbances. Also cope with the different intrinsic dynamic of the followers. assumption that external disturbance is bounded \cite{liRobustFlockingNonidentical2021}
        \item Flocking with uncertain non linea multi-agent systems. Two distributed adaptive event triggered control algorithms for leaderless and leader-follower flocking separately \cite{zouFlockingUncertainNonlinear2021}
        \item Most interesting paper for us: Flocking control, unknown nonlinear dynamics with virtual leader information. Bounded assumption on the unknown nonlinear dynamics considered, weaker than Lipschitz condition. To avoid fragmentation: construct \textbf{new potential function} based on a penalty idea when intial network is disconnected (this is interesting for us as disconnection can happen during operation!). \cite{yanFlockingMultiagentSystems2021}
        \item OK so literature has considered non-linear dynamics but what about underactuated ??
    \end{itemize}

    %%
\subsection{Underactuated work on flocking}
    \begin{itemize}
        \item Underacatuated hovercrafts circular flocking with collision avoidance. Design control in function of equation of motion. Only circular flocking \cite{hanCooperativeControlDesign2011}
        \item Leader-follower flocking of underactuated ASVs in presence of uncertain dynamics. Design a distributed adaptive flocking controller, and employ RBF NN to approximate the uncertain nonlinear dynamics in the system. Also very model based \cite{pengNeuralAdaptiveFlocking2012}
    \end{itemize}
    
    %%
 \subsection{Multiple virtual leaders}
 Finally, for our application we assume that all agents have access to their single nominal controller, which is different than most of the single virtual leader-follower flocking schemes
    \begin{itemize}
        \item Flock of autonomous agents to follow multiple virtual leaders, using only position information (still 2nd order dynamics though) \cite{suFlockingMultiAgentSystems2012}
        \item Flocking with multiple virtual leader based on connectivity preserving. Idea is to design stable control law with a navigation feedback to follow agents equipped with virtual leaders \cite{liFlockingMultiAgentSystems2016}.
    \end{itemize}

    %%
 \subsection{Conclusion:} our application blends \textbf{nonlinear, time varying dynamics} + \textbf{underactuated agents} + \textbf{multiple virtual leaders} + \textbf{uncertain dynamics}, which literature has (to the best of my knowledge not tackled all together). Difficulty is that adaptive, robust approaches to flocking might work if we were not underactuated: here sometimes there is nothing that we can do to avoid fragmentation. (Only predictive could anticipate it in advance). So our best shot is to have a potential function that allows to achieve connectivity again.
 \mwnote{We need to argue: (1) why our hierarchical approach of nominal and flocking, (2)
 If we do not include MPC, then we need to argue why not somehow (maybe b.c. too compute expensive, no formulation available?)}



